Computing Non-Archimedean Cylinder Counts in Blowups of Toric Surfaces

Counts of holomorphic disks are at the heart of the SYZ approach to mirror symmetry. In the non archimedean framework, these counts are expressed as counts of analytic cylinders. In simple cases, such as cluster varieties, these counts can be extracted from a combinatorial algorithm encoded by a scattering diagram. The relevant scattering diagram encodes information about infinitesimal analytic cylinders. In this paper, we give a formula relating counts of a restricted class of cylinders on affine log Calabi Yau surfaces to counts on a single blowup of a toric surface, using non archimedean Gromov Witten theory and a degeneration procedure parametrized by tropical data. This closed form formula constrasts with the scattering diagram approach.

==> TikZ-pictures/twig-3-valent-vertex.tex <==
\begin{tikzpicture}
\tikzstyle{length} = [<->, dotted, thin]

\draw  (-2,0) -- (-1,0) node[above] {$e'$} -- (0,0) node[above] {$v''$} -- (1,0) node[above] {$e''$} -- (2,0) ;
\draw[thin] (0,0) -- (0,-1.5) node[below] {twig} ;
 \draw[dashed] (-2,0) -- (-3,0) ;
 \draw (-3,0) -- (-4,0) node[left] {$v$} ;
 \draw[dashed] (2,0) -- (3,0) ;
 \draw (3,0) -- (4,0) node[right] {$v'$};



\end{tikzpicture}

